Fundus-R1: Training a Fundus-Reading MLLM on Public Data

Fundus imaging such as CFP, OCT and SLO is crucial for the early detection of retinal anomalies and diseases. Fundus image understanding, due to its knowledge-intensive nature, poses a challenging vision-language task. An emerging approach to addressing the task is to post-train a generic multimodal large language model (MLLM), either by supervised finetuning (SFT) or by reinforcement learning with verifiable rewards (RLVR), on a considerable amount of in-house samples paired with high-quality clinical reports. However, these valuable samples are not publicly accessible, which not only hinders reproducibility but also practically limits research to few players. In this paper, we make a novel attempt to train a reasoning-enhanced fundus-reading MLLM, termed Fundus-R1, using exclusively public datasets, wherein over 94% of the data are annotated with image-level labels only. Our technical contributions are two-fold. First, we propose a RAG-based method for composing image-specific, knowledge-aware reasoning traces. Such auto-generated traces link visual findings identified by a generic MLLM to the image labels in terms of ophthalmic knowledge. Second, we enhance RLVR with a process reward that encourages self-consistency of the generated reasoning trace in each rollout. Extensive experiments on three fundus-reading benchmarks, i.e., FunBench, Omni-Fundus and GMAI-Fundus, show that Fundus-R1 clearly outperforms multiple baselines, including its generic counterpart (Qwen2.5-VL) and a stronger edition post-trained without using the generated traces. This work paves the way for training powerful fundus-reading MLLMs with publicly available data.

==> figs/Output.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figs/Output.pdf}
\caption{Comparing MLLMs for fundus image reading}
\label{fig:pipelineeyecorer}
\end{figure*}

==> figs/case.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/Casestudy.pdf}
  \caption{Case study of \model. Green highlights denote \textcolor{cvprgreen}{retinal fidings}, while blue highlights indicate \textcolor{cvprblue}{diagnostic knowledge}.}
  \label{fig:case-study}
\end{figure}


==> figs/fail.tex <==
\definecolor{predred}{RGB}{170,30,30}
\definecolor{taggray}{RGB}{80,80,80}

\newcolumntype{L}[1]{>{\RaggedRight\arraybackslash}p{#1}}
\newcolumntype{Y}{>{\RaggedRight\arraybackslash}X}

\newcommand{\failurecase}[5]{%
\textbf{#1}\par
\vspace{0.35em}
\centering
\includegraphics[width=0.4\linewidth]{#2}\par
\vspace{0.4em}
{\raggedright\footnotesize \textbf{GT:} #3\par}
&
{\footnotesize #4}
&
{\footnotesize #5}
\\
\midrule
}

\begin{table*}[!t]
\centering

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabularx}{\linewidth}{L{0.25\linewidth} L{0.18\linewidth} Y}
\toprule
\textbf{Input} & \textbf{Choices} & \textbf{Output of Fundus-R1} \\
\midrule

\failurecase
{What type of AMD is depicted in this fundus image?}
{figs/fail/EXamd.png}
{A}
{
A. Exudative age-related macular degeneration \par
B. Nonexudative age-related macular degeneration \par
C. No any age-related macular degeneration \par
D. Polypoidal choroidal vasculopathy
}
{
\textcolor{taggray}{\texttt{<think>}} This image appears to depict a choroidal neovascular membrane (CNV), which is a hallmark feature of wet age-related macular degeneration (AMD). The CNV is characterized by the presence of abnormal blood vessels that grow beneath the retina, often leading to vision loss if left untreated. The bright, irregular area in the center of the image likely represents the CNV, which is a key diagnostic feature for wet AMD. This condition requires prompt medical intervention, typically involving laser therapy or anti-VEGF injections to prevent further damage to the retina. \textcolor{taggray}{\texttt{</think>}} \textcolor{taggray}{\texttt{<answer>}} \textcolor{predred}{wet age-related macular degeneration} \textcolor{taggray}{\texttt{</answer>}}
}

% \failurecase
% {What abnormality is presented in this fundus image?}
% {figs/fail/Blur.png}
% {C}
% {
% A. Possible glaucoma \par
% B. Vessel tortuosity \par
% C. Blur fundus \par
% D. Pathological myopia
% }
% {
% \textcolor{taggray}{\texttt{<think>}} The image exhibits a lack of clarity in the fundus structures, which is a critical visual feature. Additionally, there is an observed opacity obstructing the view of the retina and other internal ocular structures, indicating a lens-related issue. These findings suggest that light is not passing through the lens clearly, which is characteristic of cataracts. Therefore, the most plausible conclusion is that the condition corresponds to a cataract. \textcolor{taggray}{\texttt{</think>}} \textcolor{taggray}{\texttt{<answer>}} \textcolor{predred}{cataract} \textcolor{taggray}{\texttt{</answer>}}
% }

\failurecase
{What abnormality is presented in this fundus image?}
{figs/fail/DR.png}
{B}
{
A. Retinal vein occlusion \par
B. Diabetic retinopathy \par
C. Optic atrophy \par
D. Pathological myopia
}
{
\textcolor{taggray}{\texttt{<think>}} The image shows abnormality in the retinal vasculature, with evidence of venous beading and intraretinal hemorrhages. These findings are characteristic of retinal vein occlusion, as the obstruction of the central retinal vein leads to increased venous pressure and subsequent changes in the retinal vasculature. The presence of hemorrhages further supports this diagnosis, as they result from ruptured abnormal blood vessels. Therefore, the most plausible conclusion is that the condition corresponds to retinal vein occlusion. \textcolor{taggray}{\texttt{</think>}} \textcolor{taggray}{\texttt{<answer>}} \textcolor{predred}{Retinal vein occlusion} \textcolor{taggray}{\texttt{</answer>}}
}

\end{tabularx}
\caption{Failure cases of Fundus-R1 on representative fundus VQA examples.}
\label{tab:failure-cases}
\end{table*}

==> figs/hist.tex <==
\begin{figure*}[htbp]
  \centering
  \begin{subfigure}[t]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/hist/hist_overall.pdf}
    \subcaption{Overall}
  \end{subfigure}
    \begin{subfigure}[t]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/hist/hist_laterality.pdf}
    \subcaption{Laterality Classification}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/hist/hist_disease.pdf}
    \subcaption{Disease Classification}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/hist/hist_dr_grading.pdf}
    \subcaption{DR Grading}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/hist/hist_amd_grading.pdf}
    \subcaption{AMD Grading}
  \end{subfigure}
  \caption{Distribution of reasoning-text length (in words), shown overall and across key subtasks: (b) laterality classification, (c) disease classification, (d) DR grading, and (e) AMD grading.}
  \label{fig:hist}
\end{figure*}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/Prompt.tex <==

\begin{lstlisting}[caption={Prompt for direct reasoning-trace synthesis}, label={lst:direct-trace}]
You are an ophthalmology specialist. Given the question "{question}" and the image {image}, generate an English reasoning trace showing why the correct answer is {answer}.

Requirements:
- The reasoning should be grounded in the image and relevant to the question-answer pair.
- Clearly explain the evidence in the image and how it supports the answer.
- Ensure the reasoning is logically rigorous, concise, and well organized.
- Do not introduce false, hypothetical, or unsupported content.
- If any provided information is inconsistent with the target answer, treat {answer} as authoritative and produce reasoning that supports it directly, without mentioning any correction process.
- Write the reasoning as a coherent English paragraph.

Output format:
- Wrap the reasoning in <think>...</think>.
- Wrap the final answer in <answer>...</answer>.
- Output only the requested content, without any additional explanation.

Your Output:
\end{lstlisting}

\begin{lstlisting}[caption={Prompt for modality-conditioned domain knowledge extraction}, label={lst:dk-extraction}]
You are an ophthalmology expert. Given a natural-language description $desp_{y,m}$ that summarizes web-retrieved evidence for disease label "{label}" under ophthalmic image modality "{modality}", extract modality-conditioned domain knowledge as a structured JSON record.

Requirements:
- Extract only domain knowledge supported by the provided description.
- Focus on characteristic symptoms, domain criteria, and modality-specific manifestations relevant to the given label and modality.
- Organize the extracted knowledge into two categories:
  "required"   -> core findings that are essential or strongly indicative for diagnosing the condition under this modality
  "supportive" -> additional findings that may be observed and can support the diagnosis but are not essential
- Keep each item concise, clinically precise, and suitable for downstream reasoning supervision.
- Do not introduce external knowledge, unsupported inferences, or duplicated items.
- The output should reflect modality-specific ophthalmic evidence. For example, CFP findings may include lesions, hemorrhages, exudates, vascular abnormalities, or optic disc changes, whereas OCT findings may include retinal fluid, layer disruption, PED, or other structural abnormalities.
- Return the result in JSON format only.

Example output:
{
    "Moderate NPDR": {
        "required": [
            "multiple microaneurysms",
            "dot-blot intraretinal hemorrhages",
            "no evidence of neovascularization"
        ],
        "supportive": [
            "hard exudates",
            "cotton-wool spots"
        ]
    }
}

Input:
label: {label}
modality: {modality}
description: {desp_{y,m}}

Your Output:
\end{lstlisting}

\begin{lstlisting}[caption={Prompt for visual finding extraction}, label={lst:vfe-annot}]
You are an ophthalmology-aware visual inspector. Your task is to determine, for each candidate visual finding in the given vocabulary {Vocab[y,m]}, whether it is present in the input ophthalmic image{image}.

Requirements:
- Examine the image and answer each candidate finding independently.
- Map annotated regions only to the predefined controlled visual-finding vocabulary.
- For each candidate finding, output:
  1 -> present
  0 -> absent
- Base every decision strictly on visible evidence in the image and the provided annotations.
- Do not provide open-ended text, explanations, speculation, or unsupported interpretations.
- The final output must strictly follow the order of the candidate findings.

Example output:
[0, 1, 1, 0, 0, ...]

Input:
modality: {modality}
candidate findings: {Vocab[y,m]}
image: {image}

Your Output:
\end{lstlisting}

\begin{lstlisting}[caption={Prompt for synthesized reasoning-trace composition}, label={lst:reason}]
You are an ophthalmology specialist. Given the question "{question}", the visual findings {findings}, the domain knowledge {knowledge}, and the target answer {answer}, generate a single-paragraph English reasoning trace that logically supports the answer.

Requirements:
- Clearly explain how the visual findings support the answer.
- Refer to key ophthalmic evidence when relevant, such as IRF, SRF, PED, MA, DBH, VB, IRMA, RNFL, GCL, C/D, IOP, OCT, FA, and FAF.
- Ensure the reasoning is factually accurate and grounded in the provided findings and knowledge.
- Do not introduce unsupported details or hallucinated evidence.
- If there is any inconsistency among the inputs, treat {answer} as authoritative and produce reasoning that supports it directly.
- The reasoning must be written as one coherent paragraph, without bullet points, hypothetical language, or vague statements.
- Output the reasoning inside <think>...</think> and the final answer inside <answer>...</answer>.

Example:
<think>The image shows [...], including [...]. These findings indicate [...]. Therefore, the most consistent diagnosis is [...].</think><answer>{answer}</answer>

Input:
question: {question}
findings: {findings}
knowledge: {knowledge}
answer: {answer}

Your Output:
\end{lstlisting}

\begin{lstlisting}[caption={Prompt for quality control of reasoning traces}, label={lst:qc}]
You are an ophthalmology specialist. Evaluate whether the reasoning trace {traces} correctly incorporates the visual findings {findings} and the domain knowledge {knowledge}.

Requirements:
- Confirm that the reasoning accurately reflects all findings.
- Confirm that it aligns with the relevant domain knowledge.
- Confirm that the findings and knowledge are integrated coherently and support the final answer.
- Ensure that the reasoning contains no contradictions, omissions, speculation, or irrelevant details.

Output:
"1" -> the reasoning trace fully satisfies all requirements
"0" -> any requirement is missing or insufficient

Input:
traces: {traces}
findings: {findings}
knowledge: {knowledge}

Your Output:
\end{lstlisting}

\begin{lstlisting}[caption={Instruction template used for training}, label={lst:train-question}]
{question}
The reasoning process and final answer must be enclosed within <think>...</think> and <answer>...</answer> tags, respectively, i.e.,
<think> reasoning process here </think><answer> answer here </answer>
\end{lstlisting}

\begin{lstlisting}[caption={Prompt for visual finding scoring}, label={lst:train-rf}]
You are an ophthalmology specialist. Evaluate whether the reasoning trace "{traces}" correctly incorporates the visual findings {findings}.

Scoring criteria:
- low  -> major visual findings are missing, incorrectly described, or not grounded in the reasoning trace
- mid  -> the reasoning trace partially reflects the visual findings, but some findings are omitted, weakly used, or not well integrated
- high -> all visual findings are accurately reflected and coherently integrated into the reasoning trace

Output only one score: "low", "mid", or "high".

Input:
traces: {traces}
findings: {findings}

Your Output:
\end{lstlisting}

\begin{lstlisting}[caption={Prompt for domain knowledge scoring}, label={lst:train-knowledge}]
You are an ophthalmology specialist. Evaluate whether the reasoning trace "{traces}" correctly incorporates the domain knowledge {knowledge}.

Scoring criteria:
- low  -> the reasoning trace misses, misuses, or incorrectly reflects the domain knowledge
- high -> the reasoning trace accurately reflects and coherently integrates the domain knowledge

Output only one score: "low" or "high".

Input:
traces: {traces}
knowledge: {knowledge}

Your Output:
\end{lstlisting}

==> tables/RLVRhyper.tex <==

% \begin{table}[!t]
% \centering
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{1}

% \begin{tabularx}{\columnwidth}{@{}>{\raggedright\arraybackslash}p{0.24\columnwidth} >{\raggedright\arraybackslash}p{0.34\columnwidth} >{\raggedright\arraybackslash}X@{}}
% \toprule
% \textbf{Category} & \textbf{Hyperparameter} & \textbf{Value} \\
% \midrule
% \multirow{8}{=}{Optimization}
% & Optimizer & AdamW \\
% & Learning rate & $1\times10^{-6}$ \\
% & Weight decay & $1\times10^{-2}$ \\
% & Warmup ratio & 0 \\
% & Max gradient norm & 1.0 \\
% & Precision & bf16 \\
% \midrule

% \multirow{8}{=}{Actor}
% & Backbone & Qwen2.5-VL series \\
% & Vision tower trainable & True \\
% & Gradient checkpointing & True \\
% & FSDP full shard & True \\
% & CPU offload & False \\
% & Rank-0 initialization & True \\
% & Global batch size & 512 \\
% & Micro-batch size & 8, 8 \\
% \midrule

% \multirow{7}{=}{Policy regularization}
% & KL regularization & Enabled \\
% & KL penalty type & \texttt{low\_var\_kl} \\
% & KL coefficient & $1\times10^{-2}$ \\
% & Online filtering & Disabled \\
% & Padding-free training & True \\
% & Dynamic batching & True \\
% & Reward type & Sequential \\
% \midrule

% \multirow{8}{=}{Rollout}
% & Number of rollouts & 4 \\
% & Sampling temperature & 1.0 \\
% & Top-$p$ & 1.0 \\
% & Val temperature & 0.6 \\
% & Val top-$p$ & 0.95 \\
% & Val rollout number & 1 \\
% & Tensor parallel size & 2 \\
% & GPU mem utilization & 0.6 \\
% \midrule

% \multirow{4}{=}{Reference model}
% & FSDP full shard & True \\
% & CPU offload & True \\
% & Rank-0 initialization & True \\
% & Parameter offload & False \\
% \midrule

% \multirow{3}{=}{Training schedule}
% & Total epochs & 8 \\
% & Number of GPUs & 8 \\
% & Val frequency & Every 5 steps \\
% \bottomrule
% \end{tabularx}
% \caption{Training hyperparameters for the RLVR stage.}
% \label{tab:rlvr_hyperparams}
% \end{table}


\begin{table}[!t]
\centering
\caption{Training hyperparameters for the RLVR stage.}
\label{tab:rlvr_hyperparams}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1}

\begin{tabularx}{\columnwidth}{@{}>{\raggedright\arraybackslash}p{0.24\columnwidth} >{\raggedright\arraybackslash}p{0.34\columnwidth} >{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Category} & \textbf{Hyperparameter} & \textbf{Value} \\
\midrule
\multirow{8}{=}{Optimization}
& Optimizer & AdamW \\
& Learning rate & $1\times10^{-6}$ \\
& Weight decay & $1\times10^{-2}$ \\
& Warmup ratio & 0 \\
& Max gradient norm & 1.0 \\
& Precision & bf16 \\
\midrule

\multirow{5}{=}{Actor}
& Backbone & Qwen2.5-VL series \\
& Vision tower trainable & True \\
& Gradient checkpointing & True \\
& Global batch size & 512 \\
& Micro-batch size & 8, 8 \\
\midrule

\multirow{4}{=}{Policy regularization}
& KL regularization & Enabled \\
& KL penalty type & \texttt{low\_var\_kl} \\
& KL coefficient & $1\times10^{-2}$ \\
& Dynamic batching & True \\
\midrule

\multirow{8}{=}{Rollout}
& Number of rollouts & 4 \\
& Sampling temperature & 1.0 \\
& Top-$p$ & 1.0 \\
& Val temperature & 0.6 \\
& Val top-$p$ & 0.95 \\
& Val rollout number & 1 \\
& Tensor parallel size & 2 \\
& GPU mem utilization & 0.6 \\
\midrule

\multirow{3}{=}{Training schedule}
& Total epochs & 8 \\
& Number of GPUs & 8 \\
& Val frequency & Every 5 steps \\
\bottomrule
\end{tabularx}

\end{table}

==> tables/SFThyper.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{ll}
\toprule
\textbf{Hyperparameter} & \textbf{Value} \\
\midrule
Tuning type & Full-parameter tuning \\
Attention acceleration & Flash Attention \\
Optimizer & AdamW \\
Learning rate & $3\times10^{-5}$ \\
LR scheduler & Cosine \\
Warmup steps & 0 \\
Max gradient norm & 1.0 \\
Training epochs & 2 \\
Per-device batch size & 16 \\
Gradient accumulation steps & 8 \\
Precision & bf16 \\
Max sequence length & 2048 \\
Image pixel range & 1024--802816 \\
DeepSpeed & ZeRO-2 \\
\bottomrule
\end{tabular}
\caption{Training hyperparameters for the SFT stage.}
\label{tab:sft_hyperparams}
\end{table}


==> tables/casestuady.tex <==
\begin{table*}[t]
\small
\centering
\caption{Showcase of \model failure case.}
\label{tab:aokvqa-quality-showcase}
\begin{tabular}{p{0.3\linewidth} >{\raggedright\arraybackslash}p{0.68\linewidth}}
\toprule
\textbf{Questions} & \textbf{Answer} \\
\midrule
\begin{minipage}[t]{\linewidth}
What type of age-related macular degeneration is depicted in this fundus image?\\
\includegraphics[width=0.85\linewidth]{figs/blot/EXAMD.jpg}\\
GT: Exudative age-related macular degeneration
\end{minipage} 
& \begin{minipage}[t]{\linewidth}\footnotesize
\<think\>The image shows a grayish macular lesion associated with subretinal fluid, macular edema, exudation, and hemorrhages. These findings are characteristic of choroidal neovascularization, which typically presents with fluid accumulation, leakage, and bleeding beneath the retina. The presence of these features directly corresponds to the pathological process of abnormal blood vessel growth from the choroid into the subretinal space. Therefore, the most plausible conclusion is that the condition corresponds to choroidal neovascularization. \</think\>\\
\<answer\>Choroidal neovascularization \textit{</answer>}
\end{minipage} \\
\midrule
Where can the hemorrhages be found in the fundus photograph? \\
"gt": [ "Top left quadrant of the image", "Bottom right quadrant of the image", "Top right quadrant of the image"] 
& \begin{minipage}[t]{\linewidth}\footnotesize
\<think\>The image shows a grayish macular lesion associated with subretinal fluid, macular edema, exudation, and hemorrhages. These findings are characteristic of choroidal neovascularization, which typically presents with fluid accumulation, leakage, and bleeding beneath the retina. The presence of these features directly corresponds to the pathological process of abnormal blood vessel growth from the choroid into the subretinal space. Therefore, the most plausible conclusion is that the condition corresponds to choroidal neovascularization. \</think\>\\
\<answer\>Choroidal neovascularization \textit{</answer>}
\end{minipage} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/compare_with_other_models.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{\model \emph{versus} others}.
Models within each group are sorted in descending order by their average performance.
}
\label{tab:main_arch_perf}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}
>{\raggedright\arraybackslash}p{0.235\textwidth}
>{\raggedright\arraybackslash}p{0.155\textwidth}
>{\raggedright\arraybackslash}p{0.105\textwidth}
>{\raggedleft\arraybackslash}p{0.095\textwidth}
>{\raggedleft\arraybackslash}p{0.080\textwidth}
>{\raggedleft\arraybackslash}p{0.090\textwidth}
>{\raggedleft\arraybackslash}p{0.090\textwidth}
>{\raggedleft\arraybackslash}p{0.050\textwidth}
@{}}
\toprule
\textbf{Model} &
\textbf{Vision Enc.} &
\textbf{LLM} &
\textbf{\makecell[r]{Post-train Data}} &
\textbf{FunBench} &
\textbf{\makecell[r]{Omni-Fundus}} &
\textbf{\makecell[r]{GMAI-Fundus}} &
\textbf{Avg.} \\
\midrule

\multicolumn{8}{@{}l}{\textbf{Generic MLLMs}} \\
Qwen2.5-VL-3B~\cite{qwen2.5-VL}
& Qwen2.5-ViT & Qwen2.5-3B & --
& 41.0 & 66.4 & 40.4 & 49.3 \\

Qwen2.5-VL-7B~\cite{qwen2.5-VL}
& Qwen2.5-ViT & Qwen2.5-7B & --
& 51.0 & 55.6 & 52.4 & 53.0 \\

InternVL2.5-8B~\cite{chen2024expanding}
& InternViT-300M & InternLM2.5-7B & --
& 46.1 & 68.1 & 45.2 & 53.1 \\

\multicolumn{8}{@{}l}{\textbf{Medical MLLMs with SFT}} \\
HealthGPT-M3-7B~\cite{lin2025healthgptmedicallargevisionlanguage}
& CLIP ViT-L/14-336 & Phi-3-mini & 1.6M
& 52.4 & 64.0 & 50.3 & 55.6 \\

HuatuoGPT-Vision-7B~\cite{chen2024huatuogpt}
& OpenAI CLIP ViT-L/14 & Qwen2-7B & 1.3M
& 59.0 & 69.6 & 51.4 & 60.0 \\

Lingshu-7B~\cite{xu2025lingshu}
& Qwen2.5-ViT & Qwen2.5-7B & 5.1M
& 55.1 & \textbf{97.7} & 62.7 & \underline{71.8} \\

\multicolumn{8}{@{}l}{\textbf{Medical MLLMs with RLVR}} \\
MedVLM-R1~\cite{pan2025medvlm}
& Qwen2-ViT & Qwen2-2B & 600
& 46.2 & 56.3 & 40.0 & 47.5 \\

QoQ-Med-7B~\cite{dai2025qoq}
& Qwen2.5-ViT & Qwen2.5-7B & 2.6M
& 62.5 & 57.9 & 48.0 & 56.2 \\

\multicolumn{8}{@{}l}{\textbf{Fundus-reading MLLMs with SFT}} \\
FundusExpert-8B~\cite{fundusexpert}
& InternViT-300M & InternLM2.5-7B & 200K
& 48.3 & 78.4 & \textbf{76.9} & 67.9 \\

\multicolumn{8}{@{}l}{\textbf{Fundus-reading MLLMs with RLVR}} \\
OphthaReason-Intern~\cite{OphthaReason}
& InternViT-300M & Qwen2.5-1.5B & 121.5K
& 44.9 & 57.7 & 47.9 & 50.2 \\

OphthaReason-Qwen~\cite{OphthaReason}
& Qwen2.5-ViT & Qwen2.5-3B & 121.5K
& 48.8 & 62.4 & 53.0 & 54.7 \\

Med-R1-fundus~\cite{med-r1}
& Qwen2.5-ViT & Qwen2.5-3B & Undisc.
& 48.2 & 79.2 & 37.2 & 54.9 \\

\midrule
\textbf{\model{}-3B}
& Qwen2.5-ViT & Qwen2.5-3B & 80.1K
& \underline{67.1} & 79.8 & 58.5 & 68.4 \\

\textbf{\model{}-7B}
& Qwen2.5-ViT & Qwen2.5-7B & 80.1K
& \textbf{69.2} & \underline{91.1} & \underline{66.1} & \textbf{75.5} \\



\bottomrule
\end{tabular}
}

\end{table*}

==> tables/dfrf.tex <==
% =========================================================
% EyeWiki
% =========================================================
\begin{table*}[!htbp]
\centering
\caption{PubMed Central resources used for domain knowledge acquisition.}
\label{tab:domain_knowledge_pmc}
\fontsize{6.4}{7.1}\selectfont
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}

\begin{tabular}{
@{}
>{\raggedright\arraybackslash}p{0.27\textwidth}
>{\raggedright\arraybackslash}p{0.14\textwidth}
>{\raggedright\arraybackslash}p{0.55\textwidth}
@{}
}
\toprule
\textbf{Source page}
& \textbf{Category}
& \textbf{URL} \\
\midrule

EyeWiki Main Page
& Tertiary clinical
& \url{https://eyewiki.org/Main_Page} \\

Diabetic Retinopathy
& Disease
& \url{https://eyewiki.org/Diabetic_Retinopathy} \\

Diabetic Macular Edema
& Disease
& \url{https://eyewiki.org/Diabetic_Macular_Edema} \\

Diabetic Macular Ischemia
& Disease
& \url{https://eyewiki.org/Diabetic_Macular_Ischemia} \\

Age-Related Macular Degeneration
& Disease
& \url{https://eyewiki.org/Age-Related_Macular_Degeneration} \\

Choroidal Neovascularization: OCTA Findings
& Modality-specific
& \url{https://eyewiki.org/Choroidal_Neovascularization:_OCT_Angiography_Findings} \\

Optical Coherence Tomography Angiography
& Modality
& \url{https://eyewiki.org/Optical_Coherence_Tomography_Angiography} \\

Optical Coherence Tomography
& Modality
& \url{https://eyewiki.org/Optical_Coherence_Tomography} \\

OCTA and Glaucoma
& Modality-specific
& \url{https://eyewiki.org/OCT-Angiography_and_Glaucoma} \\

Macular OCT in Glaucoma
& Modality-specific
& \url{https://eyewiki.org/Macular_OCT_Imaging_in_Glaucoma} \\

SD-OCT in Glaucoma
& Modality-specific
& \url{https://eyewiki.org/Spectral_Domain_Optical_Coherence_Tomography_in_Glaucoma} \\

Vitreomacular Traction Syndrome
& Disease
& \url{https://eyewiki.org/Vitreomacular_Traction_Syndrome} \\

Macular Hole
& Disease
& \url{https://eyewiki.org/Macular_Hole} \\

Epiretinal Membrane
& Disease
& \url{https://eyewiki.org/Epiretinal_Membrane} \\

Retinal Vein Occlusion
& Disease
& \url{https://eyewiki.org/Retinal_Vein_Occlusion} \\

Branch Retinal Vein Occlusion
& Disease
& \url{https://eyewiki.org/Branch_Retinal_Vein_Occlusion} \\

Retinal Artery Occlusion
& Disease
& \url{https://eyewiki.org/Retinal_Artery_Occlusion} \\

Branch Retinal Artery Occlusion
& Disease
& \url{https://eyewiki.org/Branch_Retinal_Artery_Occlusion} \\

Retinal Detachment
& Disease
& \url{https://eyewiki.org/Retinal_Detachment} \\

Central Serous Chorioretinopathy
& Disease
& \url{https://eyewiki.org/Central_Serous_Chorioretinopathy} \\

Macular Telangiectasia
& Disease
& \url{https://eyewiki.org/Macular_Telangiectasia} \\

Hypertensive Retinopathy
& Disease
& \url{https://eyewiki.org/Hypertensive_Retinopathy} \\

Peripheral Retinal Degenerations
& Disease
& \url{https://eyewiki.org/Peripheral_Retinal_Degenerations} \\

Fundus Autofluorescence
& Modality
& \url{https://eyewiki.org/Fundus_Autofluorescence} \\

Fluorescein Angiography
& Modality
& \url{https://eyewiki.org/Fluorescein_Angiography} \\

Indocyanine Green Angiography
& Modality
& \url{https://eyewiki.org/Indocyanine_Green_Angiography} \\

Polypoidal Choroidal Vasculopathy
& Disease
& \url{https://eyewiki.org/Polypoidal_Choroidal_Vasculopathy} \\

Papilledema
& Disease
& \url{https://eyewiki.org/Papilledema} \\

Pseudopapilledema
& Disease
& \url{https://eyewiki.org/Pseudopapilledema} \\

Optic Nerve Head Drusen
& Disease
& \url{https://eyewiki.org/Optic_Nerve_Head_Drusen} \\

Demyelinating Optic Neuritis
& Disease
& \url{https://eyewiki.org/Demyelinating_Optic_Neuritis} \\

OCT in Neuro-Ophthalmology
& Modality-specific
& \url{https://eyewiki.org/Optical_Coherence_Tomography_in_Neuro-Ophthalmology} \\

Lamellar Macular Hole
& Disease
& \url{https://eyewiki.org/Lamellar_Macular_Hole} \\

Myopic Traction Maculopathy
& Disease
& \url{https://eyewiki.org/Myopic_Traction_Maculopathy} \\

Senile Retinoschisis
& Disease
& \url{https://eyewiki.org/Senile_Retinoschisis} \\

Geographic Atrophy
& Disease
& \url{https://eyewiki.org/Geographic_Atrophy} \\

Posterior Vitreous Detachment
& Disease
& \url{https://eyewiki.org/Posterior_Vitreous_Detachment} \\

Lattice Degeneration
& Disease
& \url{https://eyewiki.org/Lattice_Degeneration} \\

Horseshoe or Flap Tear
& Disease
& \url{https://eyewiki.org/Horseshoe_or_Flap_Tear} \\

Uveitic Macular Edema
& Disease
& \url{https://eyewiki.org/Uveitic_Macular_Edema} \\

Cystoid Macular Edema
& Disease
& \url{https://eyewiki.org/Cystoid_Macular_Edema} \\

Wide-Field Retinal Imaging Systems
& Modality
& \url{https://eyewiki.aao.org/Wide_field_retinal_imaging_systems} \\

Myopic CNVM
& Disease
& \url{https://eyewiki.org/Myopic_CNVM} \\

Ocular Ischemic Syndrome
& Disease
& \url{https://eyewiki.org/Ocular_Ischemic_Syndrome} \\

Optic Pits
& Disease
& \url{https://eyewiki.org/Optic_Pits} \\

Pathologic Myopia
& Disease
& \url{https://eyewiki.org/Pathologic_Myopia_(Myopic_Degeneration)} \\

\bottomrule
\end{tabular}
\caption{EyeWiki resources used for domain knowledge acquisition.}
\label{tab:domain_knowledge_eyewiki}
\end{table*}


% =========================================================
% AAO EyeNet
% =========================================================
\begin{table*}[!htbp]
\centering


\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}

\begin{tabular}{
@{}
>{\raggedright\arraybackslash}p{0.27\textwidth}
>{\raggedright\arraybackslash}p{0.14\textwidth}
>{\raggedright\arraybackslash}p{0.55\textwidth}
@{}
}
\toprule
\textbf{Source page}
& \textbf{Category}
& \textbf{URL} \\
\midrule

Nonperfusion in DR: Imaging Update
& Review
& \url{https://www.aao.org/eyenet/article/nonperfusion-in-dr-imaging-update} \\

OCTA in Diabetic Retinopathy
& Review
& \url{https://www.aao.org/eyenet/article/oct-angiography-in-diabetic-retinopathy} \\

\bottomrule
\end{tabular}
\caption{AAO EyeNet resources used for domain knowledge acquisition.}
\label{tab:domain_knowledge_eyenet}
\end{table*}


% =========================================================
% PubMed Central
% =========================================================
\begin{table*}[!htbp]
\centering


\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}

\begin{tabular}{
@{}
>{\raggedright\arraybackslash}p{0.27\textwidth}
>{\raggedright\arraybackslash}p{0.14\textwidth}
>{\raggedright\arraybackslash}p{0.55\textwidth}
@{}
}
\toprule
\textbf{Source page}
& \textbf{Category}
& \textbf{URL} \\
\midrule

DR and OCTA: Clinical Findings and Future Perspectives
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC5346852/} \\

OCTA in Retinal Vein Occlusion
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC6086221/} \\

Inner Retinal Hyperreflectivity as an Early Biomarker for CRAO
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC9299355/} \\

OCTA of the Choriocapillaris in CSC
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC6393260/} \\

Macular Telangiectasia Type 2: A Comprehensive Review
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC9553319/} \\

OCT in Papilledema and Pseudopapilledema
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC4313495/} \\

OCT in Optic Neuritis
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC3005938/} \\

Fundus Autofluorescence and Clinical Applications
& Modality review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC8358768/} \\

Near-Infrared Reflectance Imaging in Retinal Diseases
& Modality review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC8349282/} \\

OCT/OCTA Update for AMD, CSC, MacTel, and DR
& Review
& \url{https://pmc.ncbi.nlm.nih.gov/articles/PMC9858550/} \\

\bottomrule
\end{tabular}

\end{table*}

==> tables/dkexample.tex <==

\begin{table*}[t]
\centering
\caption{Examples of label- and modality-conditioned domain knowledge.}
\label{tab:dk_vf_examples}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{0.14\textwidth}
    >{\centering\arraybackslash}p{0.08\textwidth}
    >{\raggedright\arraybackslash}X
    >{\raggedright\arraybackslash}X
}
\toprule
\textbf{Label} & \textbf{Modality} & \textbf{Required VFs} & \textbf{Supportive VFs} \\
\midrule

\multirow{2}{*}{Moderate NPDR}
& CFP
& multiple microaneurysms; dot--blot hemorrhages; no evidence of neovascularization
& hard exudates; cotton--wool spots \\

& OCT
& intraretinal hyperreflective lesions consistent with hemorrhagic changes; absence of fibrovascular membrane
& mild intraretinal fluid; retinal thickening \\

\midrule

\multirow{2}{*}{Exudative AMD}
& CFP
& drusen-related macular changes; macular hemorrhage; subretinal exudative changes
& pigmentary changes; subretinal scar \\

& OCT
& subretinal fluid; intraretinal fluid; pigment epithelial detachment
& subretinal hyperreflective material; irregular retinal pigment epithelium elevation \\

\midrule

\multirow{2}{*}{Glaucoma}
& CFP
& enlarged cup-to-disc ratio; focal neuroretinal rim thinning
& optic disc hemorrhage; retinal nerve fiber layer defect \\

& OCT
& retinal nerve fiber layer thinning; ganglion cell complex thinning
& focal superior or inferior quadrant thinning \\

\midrule

\multirow{2}{*}{Diabetic Macular Edema}
& CFP
& hard exudates in the macular region; macular thickening
& microaneurysms; dot hemorrhages \\

& OCT
& intraretinal fluid; cystoid spaces; central macular thickening
& subretinal fluid; hyperreflective foci \\

\midrule

\multirow{2}{*}{Retinal Detachment}
& CFP
& elevated retina; retinal corrugation
& retinal tear; peripheral retinal folds \\

& OCT
& neurosensory retinal separation from the retinal pigment epithelium
& subretinal fluid; undulating detached retina \\

\bottomrule
\end{tabularx}

\end{table*}


==> tables/modal_select.tex <==
\begin{table}[ht]
\centering
\caption{Performance comparison on FunBench between fine-tuned Qwen2.5-VL-7B and Lingshu-7B.}
\label{tab:choose}
\begin{tabular}{lccccc}
\toprule
\textbf{MLLM} & \textbf{L1} & \textbf{L2} & \textbf{L3} & \textbf{L4} & \textbf{Mean} \\
\midrule
Qwen2.5-VL-7B & 74.8 & 98.3 & 17.3 & 60.9 & 62.8 \\
Lingshu-7B & 86.2 & 97.5 & 11.0 & 50.0 & 61.2 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/purevision.tex <==
% \begin{table}[t]
% \centering

% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Model}
% & \textbf{Lesion Recognition}
% & \textbf{Binary Condition}
% & \textbf{Multi-disease}
% & \textbf{DR Grading}
% & \textbf{AMD}
% & \textbf{Mean} \\
% \midrule

% RETFound
% & 37.0 & 64.5 & 36.3 & 49.4 & 30.7 & 43.6 \\

% DERETFound
% & 40.4 & 62.5 & 34.2 & 49.2 & 33.5 & 44.0 \\

% DINOv2-B
% & 46.9 & 76.6 & 48.1 & 56.9 & 38.4 & 53.4 \\

% DINOv2-L
% & 47.7 & 75.5 & 45.7 & 59.1 & 37.9 & 53.2 \\

% \midrule

% Qwen2.5-VL-3B
% & 36.6 & 0.3 & 34.7 & 5.6 & 13.8 & 18.2 \\

% QoQ-Med-7B
% & 13.0 & 29.4 & 39.9 & 7.3 & 14.2 & 20.8 \\

% InternVL2.5-8B
% & 46.6 & 1.2 & 41.3 & 30.9 & 32.5 & 30.5 \\

% Med-R1-fundus
% & 45.8 & 49.5 & 29.6 & 19.5 & 21.8 & 33.2 \\

% MedVLM-R1
% & 43.0 & 46.4 & 29.4 & 25.3 & 29.9 & 34.8 \\

% Qwen2.5-VL-7B
% & 34.9 & 58.3 & 41.5 & 33.3 & 26.4 & 38.9 \\

% HealthGPT-M3-7B
% & 49.4 & 54.6 & 34.2 & 37.8 & 32.3 & 41.7 \\

% OphthaReasoner-Intern-2B
% & 46.3 & 56.2 & 49.5 & 37.6 & \textbf{43.2} & 46.5 \\

% OphthaReasoner-Qwen-3B
% & 46.3 & 56.2 & 49.5 & 37.6 & \textbf{43.2} & 46.5 \\

% Lingshu-7B
% & 53.7 & 52.3 & 40.8 & 53.8 & 39.0 & 47.9 \\

% HuatuoGPT-Vision-7B
% & 54.8 & 62.2 & \underline{50.4} & 41.4 & 36.9 & 49.1 \\

% FundusExpert-8B
% & \underline{60.6} & 50.0 & \textbf{61.5} & \textbf{65.2} & 22.5 & 51.9 \\


% \rowcolor{blue!20}
% Fundus-R1-3B
% & \textbf{63.4} & \underline{79.8} & 34.4 & \underline{60.2} & 37.0 & \underline{55.0} \\
% \rowcolor{blue!20}
% Fundus-R1-7B
% & 56.0 & \textbf{80.8} & 45.6 & 57.2 & \underline{41.1} & \textbf{56.1} \\

% \bottomrule
% \end{tabular}
% }
% \caption{Comparison with pure-vision baselines. Metric: F1.}
% \label{tab:purevision}
% \end{table}

\begin{table}[t]
\centering
\caption{\textbf{MLLMs \emph{versus} pure-vision baselines}. Metric: F1.}
\label{tab:purevision}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model}
& \textbf{Lesion Rec.}
& \textbf{Binary Condition}
& \textbf{Multi-disease}
& \textbf{DR Grading}
& \textbf{AMD}
& \textbf{Avg.} \\
\midrule

RETFound
& 37.0 & 64.5 & 36.3 & 49.4 & 30.7 & 43.6 \\

DERETFound
& 40.4 & 62.5 & 34.2 & 49.2 & 33.5 & 44.0 \\

DINOv2-B
& 46.9 & 76.6 & 48.1 & 56.9 & 38.4 & 53.4 \\

DINOv2-L
& 47.7 & 75.5 & 45.7 & 59.1 & 37.9 & 53.2 \\

\midrule

Qwen2.5-VL-3B
& 36.6 & 0.3 & 34.7 & 5.6 & 13.8 & 18.2 \\

QoQ-Med-7B
& 13.0 & 29.4 & 39.9 & 7.3 & 14.2 & 20.8 \\

InternVL2.5-8B
& 46.6 & 1.2 & 41.3 & 30.9 & 32.5 & 30.5 \\

Med-R1-fundus
& 45.8 & 49.5 & 29.6 & 19.5 & 21.8 & 33.2 \\

MedVLM-R1
& 43.0 & 46.4 & 29.4 & 25.3 & 29.9 & 34.8 \\

Qwen2.5-VL-7B
& 34.9 & 58.3 & 41.5 & 33.3 & 26.4 & 38.9 \\

HealthGPT-M3-7B
& 49.4 & 54.6 & 34.2 & 37.8 & 32.3 & 41.7 \\

OphthaReasoner-Qwen-3B
& 46.3 & 56.2 & 49.5 & 37.6 & 43.2 & 46.5 \\

OphthaReasoner-Intern-2B
& 45.7 & 61.0 & 45.5 & 40.1 & \textbf{45.3} & 47.5 \\



Lingshu-7B
& 53.7 & 52.3 & 40.8 & 53.8 & 39.0 & 47.9 \\

HuatuoGPT-Vision-7B
& 54.8 & 62.2 & \underline{50.4} & 41.4 & 36.9 & 49.1 \\

FundusExpert-8B
& \underline{60.6} & 50.0 & \textbf{61.5} & \textbf{65.2} & 22.5 & 51.9 \\


\rowcolor{blue!20}
Fundus-R1-3B
& \textbf{63.4} & \underline{79.8} & 34.4 & \underline{60.2} & 37.0 & \underline{55.0} \\
\rowcolor{blue!20}
Fundus-R1-7B
& 56.0 & \textbf{80.8} & 45.6 & 57.2 & \underline{41.1} & \textbf{56.1} \\

\bottomrule
\end{tabular}
}

\end{table}

==> tables/supplytrace.tex <==
\begin{table*}[htbp]
\caption{Representative reasoning traces for selected fundus VQA examples.}
\label{tab:showcase_of_reasoning}
\setlength{\parskip}{0pt}
\setlength{\parindent}{0pt}

\newcommand{\traceheader}{
\noindent
\begin{minipage}[t]{0.4\linewidth}
\raggedright\bfseries Input VQA
\end{minipage}\hfill
\begin{minipage}[t]{0.55\linewidth}
\raggedright\bfseries Reasoning Trace
\end{minipage}\par
\vspace{0.45em}\hrule\vspace{0.6em}
}

\newcommand{\tracecase}[4]{%
\noindent
\begin{minipage}[t]{0.4\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[height=2cm]{#1}\par\vspace{0.35em}
    {\raggedright\scriptsize #2\par}
    \vspace{0.15em}
    {\raggedright\scriptsize\bfseries #3\par}
\end{minipage}\hfill
\begin{minipage}[t]{0.55\linewidth}
    \vspace{0pt}
    \raggedright \small
    \linespread{1.03}\selectfont
    #4
\end{minipage}\par
\vspace{0.5em}\hrule\vspace{0.3em}
}

\hrule height \heavyrulewidth \vspace{0.35em}

\traceheader

\tracecase
{figs/supplytrace/AH.png}
{What specific abnormalities are shown in this fundus image?}
{Asteroid hyalosis}
{%
<think>The image shows numerous white small spherical particles within the vitreous humor, distributed throughout the fundus. These particles are characteristic of asteroid bodies, which are lipid-rich structures commonly found in the vitreous. The presence of these distinct, round, refractive bodies is a key diagnostic feature. Therefore, the most plausible conclusion is that the condition corresponds to Asteroid hyalosis.</think>  <answer>Asteroid hyalosis</answer>
}

\tracecase
{figs/supplytrace/PTCR.png}
{Which abnormalities can be seen in this fundus image?}
{Post traumatic choroidal rupture}
{%
<think>The image shows a crescent-shaped yellowish/whitish subretinal streak, which is a characteristic feature of post traumatic choroidal rupture. This finding is consistent with mechanical injury to the choroid and retina, often resulting from blunt ocular trauma. The location and morphology of the streak strongly correlate with the pathophysiology of choroidal rupture. Therefore, the most plausible conclusion is that the condition corresponds to post traumatic choroidal rupture.</think><answer>Post traumatic choroidal rupture</answer>
}

\tracecase
{figs/supplytrace/IF.png}
{What kinds of lesions are represented in this fundus photograph?}
{Intraretinal Fluid}
{%
<think>The fundus photograph reveals a low reflection area within the retina, which is consistent with the presence of intraretinal fluid. This region exhibits reduced light reflectance compared to surrounding retinal structures, indicating the accumulation of fluid within the retinal layers. Such findings are characteristic of intraretinal fluid, as seen in conditions like diabetic macular edema or other retinal pathologies involving fluid leakage. The absence of other features such as hemorrhage, exudates, or pigment changes further supports this interpretation. Therefore, the most plausible conclusion is that the lesion corresponds to intraretinal fluid.</think><answer>Intraretinal Fluid</answer>
}

\tracecase
{figs/supplytrace/PCV.png}
{Which type of age-related macular degeneration is shown in this OCT image?}
{Polypoidal choroidal vasculopathy}
{%
<think>The observed features include characteristic PCV-related abnormalities, including aneurysmal polypoidal lesions and exudation. This pattern is more compatible with polypoidal choroidal vasculopathy than with typical dry or wet AMD. Thus, the correct classification is polypoidal choroidal vasculopathy.</think><answer>Polypoidal choroidal vasculopathy</answer>
}

\tracecase
{figs/supplytrace/VID.png}
{What specific abnormality is shown in this fundus image?}
{Vitreomacular Interface Disease}
{%
<think>The image shows a thickened and wrinkled retinal surface with abnormal vitreous attachment to the macula, including areas of vitreomacular adhesion and traction. The presence of a lamellar hole is also noted, along with subtle changes suggestive of epiretinal membrane formation. These findings are consistent with abnormalities at the vitreomacular interface, which can lead to mechanical stress on the macula. Therefore, the most plausible conclusion is that the condition corresponds to Vitreomacular Interface Disease.</think><answer>Vitreomacular Interface Disease</answer>
}


\end{table*}


